SASFormer: Transformers for Sparsely Annotated Semantic Segmentation

Semantic segmentation based on sparse annotation has advanced in recent years. It labels only part of each object in the image, leaving the remainder unlabeled. Most of the existing approaches are time-consuming and often necessitate a multi-stage training strategy. In this work, we propose a simple yet effective sparse annotated semantic segmentation framework based on segformer, dubbed SASFormer, that achieves remarkable performance. Specifically, the framework first generates hierarchical patch attention maps, which are then multiplied by the network predictions to produce correlated regions separated by valid labels. Besides, we also introduce the affinity loss to ensure consistency between the features of correlation results and network predictions. Extensive experiments showcase that our proposed approach is superior to existing methods and achieves cutting-edge performance. The source code is available at \url{https://github.com/su-hui-zz/SASFormer}.

==> tables/ablation2_3.tex <==
\begin{table}[!th]
\centering%
\begin{minipage}[b]{0.2\textwidth}
\centering%
\caption{Effect of different loss formations }
\label{per-lambda}
\begin{tabular}{c|c}
  \hline
  Formation & mIoU \\
  \hline
  KL  & 78.62 \\ % TreeEnergyLoss_n_21 segformer_b4_512_3_aff5.0_kl_8w.log
  \hline
  CE & 76.80 \\
  \hline
  L2 & 77.25 \\ 
  \hline
  L1 & 79.49\\
  \hline
\end{tabular}
\end{minipage}%
\hspace{3mm}%
\begin{minipage}[b]{0.2\textwidth}
\centering%
\caption{Applicability of our method}
\label{per-lambda}
\begin{tabular}{c|c|l}
  \hline
  Backbone & Ours & mIoU \\
  \hline
  \hline
  \multirow {2}{*}{Segmentor\cite{xie2021segformer}} & w/o & 72.75 \\ 
  
   ~ & w/ & 76.11(\textcolor[rgb]{1,0,0}{+3.36}) \\
  \hline
  \multirow {2}{*}{SETR\cite{zheng2021rethinking}} & w/o & 70.47\\ 
  %\hline
  ~ & w/ & 76.04(\textcolor[rgb]{1,0,0}{+5.57}) \\
  \hline
  \multirow {2}{*}{segformer\cite{xie2021segformer}} & w/o & 73.37\\ 
  %\hline
  ~ & w/ & 79.49(\textcolor[rgb]{1,0,0}{+6.12}) \\
  \hline
\end{tabular}
\end{minipage}
\end{table}




==> tables/alg.tex <==
\ref{Alg}.
\renewcommand{\thealgorithm}{1} 
\begin{algorithm}
    \caption{SASFormer algorithm} 
    \begin{algorithmic} 
        \Require A model $\mathcal{M}$ with random initialization, several different source datasets $\left \{ \mathcal{D}_s^n \right \}_{n=1}^N$, and target dataset $\mathcal{D}_t$.
        \Ensure Ranking of the results of transfer of all source datasets to target datasets when using $\mathcal{M}$.
        
        \\{$I =  epochs \ast len(dataloader) $} \quad\quad\quad//$I$ denotes the number of iterations
        % 表示迭代次数
        \For{$n = 1 \to N+1$} \quad\quad\quad//$N+1$ denotes N sources and a target
            \For{$i = 1 \to I$}
                \State Input a sample set $B_i$, $B_i\in  \mathcal{D}_s^i$ or $\mathcal{D}_t$.
                \State Computing $\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)$
                \State $\mathbb E_{i,\theta_0}[\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)]  \leftarrow ((i-1)\ast \mathbb E_{i,\theta_0}[\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)]  + \nabla \mathcal L_D( \mathcal  B_i, \theta_0)) / i$ \quad\quad\quad//The gradients obtained this time are added to the previously collected gradients and averaged 
            \EndFor
        \EndFor
        \For{$i = 1 \to N$} \quad\quad\quad//$N$ denotes the number of sources
                \State Calculate $\frac{\parallel\mathbb E_{i,\theta_0}\left [  \nabla \mathcal L_{D_t}\left ( \theta_0 \right) \right ]-\mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_s}\left ( \theta_0 \right) \right ] \parallel _2}{\parallel \mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_t}\left ( \theta_0 \right) \right ] \parallel _2\enspace \parallel \mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_s}\left ( \theta_0 \right) \right ] \parallel_2}$
        \EndFor
        \State Sort
        \State \Return Ranking
    \end{algorithmic}
\label{Alg}
\end{algorithm}

==> tables/alg_sas.tex <==
%\ref{Alg}.

\renewcommand{\thealgorithm}{1} 
\begin{algorithm}
    \caption{SASFormer algorithm} \label{Alg_SAS}
    \begin{algorithmic}
        \Require A model $\mathcal{M}$ with random initialization, several different source datasets $\left \{ \mathcal{D}_s^n \right \}_{n=1}^N$, and target dataset $\mathcal{D}_t$.
        \Ensure Ranking of the results of transfer of all source datasets to target datasets when using $\mathcal{M}$.
        
        \\{$I =  epochs \ast len(dataloader) $} \quad\quad\quad//$I$ denotes the number of iterations
        % 表示迭代次数
        \For{$n = 1 \to N+1$} \quad\quad\quad//$N+1$ denotes N sources and a target
            \For{$i = 1 \to I$}
                \State Input a sample set $B_i$, $B_i\in  \mathcal{D}_s^i$ or $\mathcal{D}_t$.
                \State Computing $\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)$
                \State $\mathbb E_{i,\theta_0}[\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)]  \leftarrow ((i-1)\ast \mathbb E_{i,\theta_0}[\nabla \mathcal L_{D}( \mathcal B_i, \theta_0)]  + \nabla \mathcal L_D( \mathcal  B_i, \theta_0)) / i$ \quad\quad\quad//The gradients obtained this time are added to the previously collected gradients and averaged 
            \EndFor
        \EndFor
        \For{$i = 1 \to N$} \quad\quad\quad//$N$ denotes the number of sources
                \State Calculate $\frac{\parallel\mathbb E_{i,\theta_0}\left [  \nabla \mathcal L_{D_t}\left ( \theta_0 \right) \right ]-\mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_s}\left ( \theta_0 \right) \right ] \parallel _2}{\parallel \mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_t}\left ( \theta_0 \right) \right ] \parallel _2\enspace \parallel \mathbb E_{i,\theta_0}\left [ \nabla \mathcal L_{D_s}\left ( \theta_0 \right) \right ] \parallel_2}$
        \EndFor
        \State Sort
        \State \Return Ranking
    \end{algorithmic}

\end{algorithm}
%\end{document}
